Insights from Game Theory into the Impact of Smart Balancing on Power System Stability

Smart balancing, also called passive balancing, is the intentional introduction of active power schedule deviations by balance responsible parties (BRPs) to receive a remuneration through the imbalance settlement mechanism. From a system perspective, smart balancing is meant to reduce the need for, and costs of, frequency restoration reserves (FRR), but it can also cause large oscillations in the FRR and jeopardize the system stability. Using a dynamic control area model, this work defines a 2x2 game in which two BRPs can choose to perform smart balancing. We study the impact of time delay, ramp rates, and pricing mechanisms on Nash equilibria and Experience-weighted Attraction (EWA) learning. It is found that, even in an idealized setting, a significant fraction of games in a learned equilibrium results in an overreaction relative to the baseline disturbance, creating an imbalance in the opposite direction. This suggests that the system stability risks are inherent to smart balancing and not a question of implementation. Recommendations are given for implementation choices that can reduce (but not eliminate) the risk of overreactions.

==> Tables/overreactionProbabilities.tex <==
\begin{tabular}{llcccccc}
\toprule
 $T_\mathrm{game}$ & $\mathrm{d}P/\mathrm{d}t$ & \multicolumn{3}{c}{DE-pricing} & \multicolumn{3}{c}{NL-pricing} \\
$\left[\mathrm{min}\right]$ & $\left[\mathrm{\%/min}\right]$ & NE \cref{eq:mixedNE} & $\beta\!=\!1$ & $\beta\!=\!\infty$ & NE \cref{eq:mixedNE} & $\beta\!=\!1$ & $\beta\!=\!\infty$ \\
\midrule
1 & 400 & 14.4 & 15.6 & 0.1 & 13.0 & 14.3 & 0.1 \\
 &  &  & (9.1) & (3.6) &  & (9.2) & (3.3) \\
1 & 20 & 22.1 & 17.5 & 0.2 & 19.4 & 15.4 & 0.2 \\
 &  &  & (9.5) & (4.3) &  & (9.7) & (4.7) \\
5 & 400 & 38.4 & 22.1 & 0.3 & 25.0 & 16.4 & 0.2 \\
 &  &  & (10.2) & (5.1) &  & (10.3) & (4.5) \\
5 & 20 & 44.9 & 23.9 & 0.5 & 28.1 & 17.6 & 0.4 \\
 &  &  & (10.3) & (7.3) &  & (10.3) & (5.9) \\
10 & 400 & 49.0 & 24.9 & 0.2 & 34.8 & 19.2 & 0.3 \\
 &  &  & (10.2) & (4.3) &  & (10.5) & (5.4) \\
10 & 20 & 50.4 & 25.5 & 0.1 & 50.4 & 23.1 & 0.1 \\
 &  &  & (9.9) & (3.3) &  & (11.2) & (3.8) \\
\bottomrule
\end{tabular}


==> glossary.tex <==
%\newacronym{tso}{TSO}{Transmission System Operator}
%\newacronym{ca}{CA}{Control Area}
%\newacronym[\glslongpluralkey={Balance Responsible Parties}]{brp}{BRP}{Balance Responsible Party}
%\newacronym{ace}{ACE}{Area Control Error}
%\newacronym{isp}{ISP}{Imbalance Settlement Period}
%\newacronym{frr}{FRR}{Frequency Restoration Reserve}
%\newacronym{afrr}{aFRR}{automatic Frequency Restoration Reserve}
%\newacronym{mfrr}{mFRR}{manual Frequency Restoration Reserve}
%\newacronym{fcr}{FCR}{Frequency Containment Reserve}
%\newacronym{bsp}{BSP}{Balancing Service Provider}
%\newacronym{nrt}{NRT}{Near Real-Time}
%\newacronym{kpi}{KPI}{Key Performance Indicator}
%\newacronym{gcc}{GCC}{German Grid Control Cooperation}
%\newacronym{nl}{NL}{the Netherlands}
%\newacronym{de}{DE}{Germany}

\newacronym{tso}{TSO}{transmission system operator}
\newacronym{ca}{CA}{control area}
\newacronym[\glslongpluralkey={balance responsible parties}]{brp}{BRP}{balance responsible party}
\newacronym{ace}{ACE}{area control error}
\newacronym{isp}{ISP}{imbalance settlement period}
\newacronym{frr}{FRR}{frequency restoration reserve}
\newacronym{afrr}{aFRR}{automatic frequency restoration reserve}
\newacronym{mfrr}{mFRR}{manual frequency restoration reserve}
\newacronym{fcr}{FCR}{frequency containment reserve}
\newacronym{bsp}{BSP}{balancing service provider}
\newacronym{nrt}{NRT}{near real-time}
\newacronym{kpi}{KPI}{key performance indicator}
\newacronym{gcc}{GCC}{German grid control cooperation}
\newacronym{nl}{NL}{the Netherlands}
\newacronym{de}{DE}{Germany}
\newacronym[\glslongpluralkey={Nash equilibria}]{ne}{NE}{Nash equilibrium}
\newacronym{fp}{FP}{fixed point}
\newacronym{ewa}{EWA}{experience-weighted attraction}

==> keywords.tex <==
smart balancing, power system stability, game theory, experience-weighted attraction, frequency restoration reserve, imbalance settlement,  passive balancing
